TheoremQA: A Theorem-driven Question Answering dataset

The recent LLMs like GPT-4 and PaLM-2 have made tremendous progress in solving fundamental math problems like GSM8K by achieving over 90% accuracy. However, their capabilities to solve more challenging math problems which require domain-specific knowledge (i.e. theorem) have yet to be investigated. In this paper, we introduce TheoremQA, the first theorem-driven question-answering dataset designed to evaluate AI models' capabilities to apply theorems to solve challenging science problems. TheoremQA is curated by domain experts containing 800 high-quality questions covering 350 theorems (e.g. Taylor's theorem, Lagrange's theorem, Huffman coding, Quantum Theorem, Elasticity Theorem, etc) from Math, Physics, EE&CS, and Finance. We evaluate a wide spectrum of 16 large language and code models with different prompting strategies like Chain-of-Thoughts and Program-of-Thoughts. We found that GPT-4's capabilities to solve these problems are unparalleled, achieving an accuracy of 51% with Program-of-Thoughts Prompting. All the existing open-sourced models are below 15%, barely surpassing the random-guess baseline. Given the diversity and broad coverage of TheoremQA, we believe it can be used as a better benchmark to evaluate LLMs' capabilities to solve challenging science problems. The data and code are released in https://github.com/wenhuchen/TheoremQA.

==> gpt4_accuracy_on_existing_dataset.tex <==
\begin{tikzpicture}
\centering
\begin{axis}[
    ybar,
    %enlargelimits=0.15,
    %ylabel={Accuracy},
    height=2.5in, 
    symbolic x coords={GSM8K, ASDiv, Math23K, SVAMP, AQuA, FinQA, ScienceQA},
    xtick=data,
    x tick label style={rotate=60,anchor=east},
    nodes near coords,
    nodes near coords align={vertical},
    ymin=0.5, ymax=1.1,
    % xlabel={Existing Datasets},
    bar width=10pt
]
\addplot coordinates {
    (GSM8K, 0.92)
    (ASDiv, 0.95)
    (Math23K, 0.94)
    (SVAMP, 0.94)
    (AQuA, 0.75)
    (FinQA, 0.76)
    (ScienceQA, 0.90)
};
\end{axis}
\end{tikzpicture}
